GPS-Based Geolocation of Consumer IP Addresses

This paper uses two commercial datasets of IP addresses from smartphones, geolocated through the Global Positioning System (GPS), to characterize the geography of IP address subnets from mobile and broadband ISPs. Datasets that ge olocate IP addresses based on GPS offer superlative accuracy and precision for IP geolocation and thus provide an unprecedented opportunity to understand both the accuracy of existing geolocation databases as well as other properties of IP addresses, such as mobility and churn. We focus our analysis on large cities in the United States. After evaluating the accuracy of existing geolocation databases, we analyze the circumstances under which IP geolocation databases may be more or less accurate. We find that geolocation databases are more accurate on fixed-line than mobile networks, that IP addresses on university networks can be more accurately located than those from consumer or business networks, and that often the paid versions of these databases are not significantly more accurate than the free versions. We then characterize how quickly subnets associated with fixed-line networks change geographic locations, and how long residential broadband ISP subscribers retain individual IP addresses. We find, generally, that most IP address assignments are stable over two months, although stability does vary across ISPs. Finally, we evaluate the suitability of existing IP geolocation databases for understanding Internet access and performance in human populations within specific geographies and demographics. Although the median accuracy of IP geolocation is better than 3 km in some contexts, we conclude that relying on IP geolocation databases to understand Internet access in densely populated regions such as cities is premature.

==> _ <==
#!/bin/bash

mkdir -p jtex && cd jtex

pop_notes -s -p  173 -q ~/papers/internet/2001_padmanabhan_geoping_geocluster.pdf
pop_notes -s -p    1 -q ~/papers/internet/2002_spring_rocketfuel_geo.pdf
pop_notes -s -p  153 -q ~/papers/internet/2005_freedman_feamster_geographic_locality_ip_prefixes.pdf
pop_notes -s -p 1219 -q ~/papers/internet/2006_gueye_constraint_based_geolocation.pdf
pop_notes -s -p   71 -q ~/papers/internet/2006_katz-basett_geolocation_delay_and_topology.pdf
pop_notes -s -p  237 -q ~/papers/internet/2007_imprecision_of_block_geolocation.pdf
pop_notes -s -p    1 -q ~/papers/internet/2007_wong_octang_geolocation_negative.pdf
pop_notes -s -p  171 -q ~/papers/internet/2010_erikkson_barford_learning_based_geolocation.pdf
pop_notes -s -p    1 -q ~/papers/internet/2010_gill_geolocation_circumvention.pdf
pop_notes -s -p   53 -q ~/papers/internet/2011_poese_uhlig_ip_geolocation_unreliable.pdf
pop_notes -s -p 2044 -q ~/papers/internet/2011_shavitt_geolocation_study.pdf
pop_notes -s -p    1 -q ~/papers/internet/2011_wang_street_level_geolocation.pdf
pop_notes -s -p    2 -q ~/papers/internet/2012_eriksson_barford_posit_lightweight_geolocation.pdf
pop_notes -s -p  123 -q ~/papers/internet/2012_zi_geolocations_of_millions_of_addresses.pdf
pop_notes -s -p  381 -q ~/papers/internet/2013_li_geolocation_moderately_connected.pdf
pop_notes -s -p  463 -q ~/papers/internet/2017_gharaibeh_router_geolocation.pdf
pop_notes -s -p    1 -q ~/papers/internet/2018_ovidiu_geolocation_reverse_dns.pdf


cat lit_rev_overview > ipgeo_lit_rev
cat jtex/*/* | sed 's/&/\\&/g' >> ipgeo_lit_rev

cat \
    jtex/internet/2001_padmanabhan_geoping_geocluster \
    jtex/internet/2002_spring_rocketfuel_geo \
    jtex/internet/2005_freedman_feamster_geographic_locality_ip_prefixes \
    jtex/internet/2006_gueye_constraint_based_geolocation \
    jtex/internet/2006_katz-basett_geolocation_delay_and_topology \
    jtex/internet/2007_imprecision_of_block_geolocation \
    jtex/internet/2007_wong_octang_geolocation_negative \
    jtex/internet/2010_erikkson_barford_learning_based_geolocation \
    jtex/internet/2010_gill_geolocation_circumvention \
    jtex/internet/2011_poese_uhlig_ip_geolocation_unreliable \
    jtex/internet/2011_shavitt_geolocation_study \
    jtex/internet/2011_wang_street_level_geolocation \
    jtex/internet/2012_eriksson_barford_posit_lightweight_geolocation \
    jtex/internet/2012_zi_geolocations_of_millions_of_addresses \
    jtex/internet/2013_li_geolocation_moderately_connected \
    jtex/internet/2017_gharaibeh_router_geolocation \
    jtex/internet/2018_ovidiu_geolocation_reverse_dns \
    | sed 's/&/\\&/g' >> ipgeo_lit_rev 
    
echo "\\bibliographystyle{bibulous}" >> ipgeo_lit_rev
echo "\\bibliography{sources}" >> ipgeo_lit_rev

cat ../../internet/sources.bib > sources.bib

##  jtex -p -d -i ipgeo_lit_rev
##  bibulous ipgeo_lit_rev.aux
##  pdflatex ipgeo_lit_rev
##  pdflatex ipgeo_lit_rev



==> geolocation <==
^T: Heterogeneity in the Localizability of IP Addresses
^H: \usepackage[sort]{natbib}
^H: \usepackage{booktabs}
^H: \graphicspath{{figs/}}
^H: \captionsetup{width=\textwidth}


This paper leverages a large commercial dataset 
  of IP addresses from consumer smartphones, geolocated through GPS, 
  to evaluate existing geolocation databases.
While most of the recent literature takes for granted
  that IP addresses have meaningful locations,
  consumer addresses are usually assigned dynamically.
The time scale for reassignment varies, 
  but IP addresses used on cellular networks in particular
  may be reassigned very rapidly over a large area.
Mobile and fixed broadband infrastructures differ fundamentally,
  and this difference is reflected in the localizability of devices on those networks.
We therefore present and analyze heterogeneity in the extent to which 
  individual addresses or address blocks can be associated with a fixed location.
Our work is distinguished by our large sample of consumer devices and 
  by its superlative geographic precision.
These data allow us to study geolocalization performance
  at the level of neighborhoods within cities.

The paper begins with a brief review of 
  existing literatures and the data.
We then present basic facts about IP geolocation accuracy
  and then analyze when it does and does not work.
Specifically,
  we show that physically small subnets can be geolocated fairly accurately,
  and that subnets' movement over time is slow.
Before concluding, we interpret our results in the context of 
  research on human populations and privacy.

> Existing Literatures 

Accurate geolocalization of IP addresses is a classic networking problem
  with both an active academic literature and vibrant commercial applications.
Geolocation is used to
  specialize search results and target advertising.
It can be used to present relevant content (like weather),
  or change its presentation (language localization).
Legally, it is used to deliver content (rights management),
  abide by local laws (gambling or taxes), and 
  aid in enforcement (determining jurisdictions or collecting evidence).
In security contexts, government and commercial entities use it for
  for counter-terrorism, attack attribution,
  monitoring access to private networks, and flagging potential fraud.
It facilitates operations and site reliability (packet loss from a location), and 
  informs infrastructure investments by both industry and policymakers.
And it is used for computer science research~--
  for instance on the structure and graph parameters of networks.

An application that is less recognized in past work, 
  and which initially motivated the present one, 
  is \emph{social} science research.
It is popular (or tiresome) to note the potential of “big data”
  as a lens on human behaviors and interactions.
As modern society is increasingly mediated through the Internet,
  many of our interactions are labelled~-- at some point~-- by IP address.
Server logs and speedtests, for instance, 
  show who accesses resources and the quality of their connection.
This allows aggregate statistics or time trends,
  but to associate these behaviors or experienced network conditions
  with a population, we need a “dictionary” to translate
  from the Internet space to human space.
IP geolocation with Census tract-scale precision would make that link.

Past work on geolocalization can be split roughly into three approaches,
  all formulated as Athena from the head of Zeus,
  by \cite{2001_padmanabhan_geoping_geocluster}.
Their IPGeo work compared the complementary strengths of 
  active latency measurements (GeoPing),
  active traceroutes paired with DNS hints (GeoTrack), and 
  static databases of outside information (GeoCluster).
Over time, each of these approaches has evolved.
Padmanabhan and Subramanian 
  concluded that database-driven methods held the greatest promise.
Commercial firms have heeded this advice, 
  with distributable-databases built with proprietary methods that 
    include both registry and geolocation data and active methods.
On the other hand, academic work has tended to focus
  on active and DNS-based measurements.

Starting with DNS,
  \cite{2002_spring_rocketfuel_geo}
  developed techniques in their Rocketfuel project to 
  maximize the new information of each traceroute, 
  by minimizing redundancy and working to ensure that each path will traverse its target ISP.
Their subsequent approach to DNS hint identification was largely manual~-- 
  ``browsing through the list of router names''~-- 
  but the resultant \texttt{undns} tool has proven influential and enduring.
A few years later, \cite{2005_freedman_feamster_geographic_locality_ip_prefixes} extended \texttt{undns}' coverage.
Both of these projects were driven by fundamental network research questions~--
  the network properties of large ISPs and the efficiency of block assignments in BGP routing tables~--
  and underscore the academic and practical need for these measurements.
More recently,
  \cite{2018_ovidiu_geolocation_reverse_dns} made a systematic effort 
  to itemize all possible DNS city name hints and 
  finalize location decisions through a compelling machine learning setup.
Like IPGeo, the authors relied on a large dataset from Microsoft
  for their ground truth -- this time Bing instead of Hotmail.

In the latency-based space, 
  \cite{2006_gueye_constraint_based_geolocation} and 
  \cite{2006_katz-basett_geolocation_delay_and_topology}
  introduced constraint-based geolocation (CBG) and topology-based geolocation (TBG).
CBG is essentially the intersection of several latency-derived distance buffers, 
  while TPG also localizes intermediate hosts
  so that targets can be constrained by their relation to passive landmarks rather than just active probes.
Subsequently, Octant \citep{2007_wong_octang_geolocation_negative}
  incorporated both positive \emph{and negative} constraints
  (the IP address is \emph{not} within a certain radius).

In addition to this ``geometric'' aproach
  are several statistical strategies.
\citeauthor{2010_erikkson_barford_learning_based_geolocation} developed
  first a Bayesian approach \citeyearpar{2010_erikkson_barford_learning_based_geolocation} and 
  then a likelihood-driven choice among possibilities with the CBG-derived regions 
  \citeyearpar{2012_eriksson_barford_posit_lightweight_geolocation}.
\cite{2009_youn_kde_geolocation} and \cite{2010_arif_mle_geolocation}
  present strategies using kernel density and maximum likelihood estimation, respectively.
It is also possible to constrain location
  from the covariance matrix of latency measurements with locations.

Notable in \citeauthor{2010_erikkson_barford_learning_based_geolocation}'s Bayesian work
  is the insight that outside information can help constrain or inform geolocation.
They used population as a measure of places' importance,
  as have later researchers
  \citep{2018_ovidiu_geolocation_reverse_dns}.
Other forms of information help as well.
In trace-based work reminiscent of TPG,
  \cite{2011_wang_street_level_geolocation} performed extensive 
  webscraping and analyis to identify and confirm businesses with locally-hosted sites 
  that they could “enlist” as passive landmarks.
They used those landmarks to identify the locations of routers near the geolocation target.

Scalability has long been a limitation of active measurements.
Since locations are most-constrained by the closest locations,
  \cite{2012_zi_geolocations_of_millions_of_addresses} developed methods
  to prioritize measurements from nearby hosts, effectively by localizing avatars from subnets.
Alternatively, \cite{2013_li_geolocation_moderately_connected}
  “flip” the standard infrastructure of active geolocation with GeoGet:
  the targets to be localized measure the latency themselves, through javascript, 
  rather than generating pings through an API.
This reduces the number of servers and traffic required,
  and it is also helpful since clients' devices or networks 
  may fail to respond to pings or complete traceroutes.

These advances notwithstanding,
  commercial geolocation tends to be implemented through databases.
Databases are inexpensive to distribute and
  can aggregate historical observations across many sources.
The leading services~--
  MaxMind, IP2Location, Akamai, or NetAcuity~
  use proprietary methods.
A number of papers assess the performance of these databases,
  ground-truthing with the preceding active methods \citep{2007_imprecision_of_block_geolocation},
  points-of-presence paired with routing tables from a large ISP \citep{2011_poese_uhlig_ip_geolocation_unreliable},
  DNS look-ups paired with ground truth rules from domain operators \citep{2017_gharaibeh_router_geolocation},
  from RIPE ATLAS built-in measurements, or PlanetLab nodes,
  or against each-other, sometimes with a majority logic applied.
It is worth noting that the databases are themselves 
  often taken as the ground-truth for latency-based measurements,
  sometimes with a sort of majority logic.
\cite{2011_shavitt_geolocation_study}
  employ that strategy in evaluating the databases themselves, 
  but also focus on \emph{consistency}
  among addresses determined to share a point-of-presence, 
  based on an earlier algorithm \citep{2012_feldman_pop_geolocation}. 
Similarly, \cite{2011_huffaker_geocompare}
  assess the agreeement of country determinations and distances from a centroid, 
  from majority votes (supplemented by PlanetLab ground-truth and limited RTT measurements).

So what is the verdict?
On the whole, both the formal literature and ``popular wisdom"
  paint a fairly pessimistic picture of geolocation performance.
Early academic projects quote median accuracy 
  at 25~km in Western Europe and 100~km in the United States.
On the commercial side, 
  \cite{2011_poese_uhlig_ip_geolocation_unreliable}
  quote median accuracies 
  between tens and hundreds of kilometers
  for MaxMind and IP2Location.
Other early works present CDFs with ranges stretching
  hundreds or thousands of kilometers, 
  suggestive of the scale. \citep{2011_shavitt_geolocation_study}
\citeauthor{2017_gharaibeh_router_geolocation}
  present results for routers in particular, 
  with median accuracies betweeen 10~km for NetAcuity and 1000~km for IP2Location, 
  sandwiching the free and paid versions of MaxMind.
More recently, \citeauthor{2018_ovidiu_geolocation_reverse_dns}
  presented medians between 10 and 30~km, depending
    on the sample and service.
They present results in 10~km bins, and do not differentiate
  performance at the very bottom of the range.

A persistent though somewhat more subtle current
  of the literature has explored the physical
  structure of the Internet and its relation to geolocation accuracy.
\citeauthor{2001_padmanabhan_geoping_geocluster} anticipated
  even this line of work~-- 
  the interplay between network infrastructure and geolocation accuracy~--
  back in 2001.
They noted the impact
  of the geographical concentration of AOL's login nodes on accuracy,
  and showed that clusters of addresses that were physically larger
  were associated with poorer performance for the GeoCluster (database) method.
This point was echoed by \citeauthor{2007_imprecision_of_block_geolocation}
  in \citeyear{2007_imprecision_of_block_geolocation}.
Similarly, \cite{2005_freedman_feamster_geographic_locality_ip_prefixes} 
  measured the physical scale of autonomous systems,
Later, \cite{2016_gharaibeh_geo_ip_colocality} 
    probed the common assumption of databases
    that /24 subnets are colocalized.
Those papers show that 
  systems, subnets, and BGP blocks
  are often physically quite large. 
We aim to identify the circumstances when they are large or small.
An important refinement of \citeauthor{2011_huffaker_geocompare}'s work
  was to decompose accuracy according to carriers' network role;
  we continue that impulse here, contrasting accuracy
  on commercial ISPs, large companies, and universities.
Specifically, we categorize addresses by CIDRs ``Doing-Business As" names;
  no paper that we are aware of has investigated performance among providers,
  let alone in the modern, mobile era.
The fact that mobile and wired infrastructures
  differ is obvious once stated,
  but both data and discussion of this fact 
  have been absent from the literature.

Past work on evaluation has tended to rely either
  on active measurements of somewhat coarse precision
  or else on a fairly consistent set of (unrepresentative) benchmarks: 
  PlanetLab sites and university clusters.
The present dataset is, no doubt, also peculiar~-- 
  a non-random sample of mobile devices~-- 
  but this view from the access network is critical.
It is indicative a large set of realistic consumer geolocation targets.
The Global Positioning System (GPS) 
  has long served as a counterpoint to IP geolocation, 
  both as a benchmark of accuracy and as an analog in multilateration.
Historically,
  its deployment and use for Internet measurement 
  felt impossibly far off
  \citep{2006_katz-basett_geolocation_delay_and_topology,2010_erikkson_barford_learning_based_geolocation,2012_eriksson_barford_posit_lightweight_geolocation},
  but the future has now arrived.

This paper extends previous work
  thanks chiefly to its large sample of
  consumer smartphone locations on diverse networks.
The primary dataset was provided by Unacast.
Similar datasets are readily available
  for commercial applications and academic research.
We exploit this sample to understand heterogeneity in address localizability.
In an appendix,
  we confirm our basic results on a smaller, Chicago-only 
  sample of GPS-located speedtests from Ookla.
In contrast to previous work, which has 
  tended to question the overall reliability of geolocation even at country-level accuracy,
  we argue that it works fairly well in predictable and well-defined contexts.
Still, the imperfect accuracy and context-specific performance 
  limit applications in academic research.


> The Data

>> GPS Smartphone Location Data

The dataset that we have received from Unacast contains 
  clusters of GPS locations reported by mobile devices,
  along with timestamps and unique, anonymous identifiers.
Unacast aggregates multiple location data streams from other firms;
  they perform extensive data validation, deduplication, and processing
    on those streams.
The exact applications that generate locations are not provided.\footnote{
  Data are collected in accordance with local laws and opt-out policies (GDPR), 
    and analyzed with IRB exemption from the University of Chicago.}

The median reported GPS location accuracy is 17~m.
A small fraction of data (0.3\%) are recorded 
  with only two decimal points of coordinate precision,
  corresponding to about 1~km;
  we exclude them from subsequent analyses.\fnote{Re-run with this update!}
As discussed below, an IP address
  is reported for about half of clusters.
The full dataset thus offers IP addresses
  recorded at 700 million locations.
Data are provided for August through October 2020,
  within a 40~mile buffer of 
  three major American cities:
  New York, Chicago, and Philadelphia.

Individual locations 
  are clustered using Unacast's proprietary algorithm.
That algorithm uses machine learning to account 
  for variation in physical scale among locations:
    a mall is larger than a coffee shop or a home.
Clusters are labelled according to their durations,
  which are also reported.
Locations recorded during movement 
  are labelled as \texttt{TRAVEL}.
See the Appendix for a breakdown of cluster types.
This clustering reduces the data volume
  by a factor of 20 while retaining most of the information.
The raw, un-clustered data often cannot be relicensed.

The clustering does entail some subtlety:
  a single physical location and IP address is reported per cluster,
  so that the centroid of a \texttt{TRAVEL} cluster may not exactly
    coincide with the moment that the reported IP address was used.
Indeed, the physical location of a consumer IP address is often not fixed;
  for instance, consumers can roam freely through their home while connected to their WiFi.
In practice, individual IP addresses
  are recorded at many physical locations~--
  and these locations may be close or distant from each other.

We use night-time clusters as a proxy 
  to concentrate analysis on residential broadband.
We define these clusters as those that intersect
  the time-period period from midnight to 6am of any day.
Clusters that last into the night represent 
  just 4.8\% of clusters but 27\% raw location reports, or \emph{bumps}.
Across devices, 16\% have at least one night-time cluster,
  but those 16\% of devices generate a majority of the dataset:
  84\% of clusters and 92\% of bumps.
In short, weighted by data volume,
  most devices have observations at times 
  when they can reasonably be assumed at home.
Focussing on that set of devices (with night-time location reports),
  the ratio of devices to the population of the study region is about 1 to 20.

To decompose localizability of addresses by network type,
  we also identify ISPs.
Each address is associated with its /24 subnet,
  whose organization is retrieved from the ARIN whois registry.% \footnote{On what date.}
If the prefix size exceeds 24 on IPv4 or 48 on IPv6,
  we follow the link to the “parent” network.
This strategy is philosophically similar to an ASN lookup, 
  and differs in practice primarily in superior coverage of 
  Department of Defense NIC, wireless carriers, and foreign NICs.
The ASN lookup also “fractures” organizations 
  like small city governments or businesses from their providers.
We associate large and common organizations with standardized “Doing Business As” (DBA) names,
  taking particular care to capture the major ISPs in each market (Comcast, Charter, etc.).
We separate AT\&T's and Verizon's mobile broadband from their fixed offerings
  based on the words ``Mobility" or ``Wireless" in the organization name.
This may not be a perfect division:
  ``Verizon Business" and ``AT\&T Services" may include mobile offerings,
  but examining the ASN tables suggests this is not their primary use.

These procedures also identify large companies and institutions, in particular, universities.
We flag addresses from universities with at least ten thousand students,
  and Fortune 100 companies.
Universities clusters are ``classic" targets for academic work on geolocation,
  since they have have meaningful and well-known locations, 
  but they are not representative of the consumer space.
We exclude ISPs, including Google, from the Fortune 100 set.
We retain IANA special use and non-ARIN addresses,
  to perform cross-checks on the underlying data.
Ultimately, each address is associated with a single DBA name for analysis.

>> Geolocation Databases and Distance Calculations

We obtain the free and subscription versions of the less-expensive geolocation databases:
  MaxMind and IP2Location, for August 1, 2020.
Per the license,
  geolocation is peformed only for the single month of data following that date.
The NetAcuity and Akamai geolocation services, 
  which are much more expensive, are not included in this work.
Using these databases, we geolocate each IP address recorded in the GPS sample.
We then measure the Vincenty distance (on the ellipsoid of Earth)
  from each IP-geolocated point to the location recorded by the GPS-enabled device.
For most of what follows, we take the GPS as the “ground truth” and call the entire
  distance the “accuracy” or “error.”
Since the database providers acknowledge their limited resolution 
  and in certain cases quantify it accurately, 
  this language is perhaps unfair:
  it is different for a database to acknowledge a location as unknown 
    or indeterminate (as in reserved, private addresses) than to be “wrong” about the location.
Semantics aside,
  the balance of this work tabulates distances with respect to the ground truth
  and seeks to explain their heterogeneity.

> Results

>> Are GPS data a credible ground truth of IP address locations?

Location data have attracted increased attention 
  throughout the Coronavirus pandemic, 
  as a lens on human mobility and social distancing.
The accuracy of these locations is Unacast's core business, and 
  they dedicate enormous resources to validating and maintaining their incoming data streams.
The data stream of IP addresses is not the primary one,
  and it has seen less global attention and validation.
We begin with a few ``sanity'' checks before proceeding to the core analyses.

The share of data reporting IANA 
  reserved or private addresses low, 0.5\%,
  and the share of addresses associated with foreign Internet registries
  totals just 0.2\% (breakdown shown in the Appendix).
The traffic observed is overwhelmingly IPv4, at 99.6\%.
We also expect that the clustering procedures could affect 
  the “compatibility” of the IP address and GPS location.
For example, if a GPS location is recorded when no network is available,
  it may be subsequently \emph{reported} at a different physical location
  where an IP address can be obtained.
We would expect this effect to be most severe for \texttt{TRAFFIC} clusters,
  as previously discussed.
Night-time clusters tend to be longer and may therefore be more precisely determined, and
  geolocation on mobile networks performs poorly in general (as shown below).
We therefore limit this analysis to daytime pings on a single fixed network -- Comcast.
As expected, we observe that accuracy is lower for travel than non-travel data, 
	but the difference in medians is only 3.5\% for IP2Location and 6.0\% for MaxMind.
As can be seen in the Appendix, the cumulative distribution functions for 
  for travel and non-travel clusters are in fact quite close across their entire range.

>> Which database provides the lowest error in location?

The practical question is which database to use, 
	and how well it should be expected to perform.
The simple answer is that MaxMind\fnote{paid?} is best.
The traditional way of reporting this is the median error,
	which is 27~km for MaxMind and 46.6~km for IP2Location.
Other quantiles are shown in Table~\ref{tab:distance_quantiles_by_db}.
The empirical Cumulative Distribution Function (CDF)
  of distances by city and database reported for each database in Figure~\ref{fig:cdf_by_city}.\footnote{Compare paid and free versions?  Compare to their own account of their city-level accuracy.}
Here and below, ``city" is taken to mean the city itself along with the 40-mile 
	buffer around it.
Since it is just 46 miles from Staten Island to North Philadelphia,
	some data are included in the curves for both New York and Philadelphia.

\input{tabs/distance_quantiles_by_db.tex}

cdf_by_city.pdf:0.6 Cumulative distribution function by geolocation database and city. Colors reference databases, and line styles show cities.  \label{fig:cdf_by_city}

>> Under what circumstances is IP geolocation reliable?

These basic results mask extreme but unsurprising heterogeneity.
Figure~\ref{fig:cdf_by_city} already shows that geolocation performs
	better in New York than Chicago, and better in Chicago than Philadelphia.
But the largest source of heterogeneity stems from providers,
	which deploy different physical infrastructures
	(and serve different cities).

cdf_cities_dbs.pdf:1.0 Geolocation performance by city, database, and ISP. ISPs are shown by their ``brand" colors, according to the whois database, which leaves the Sprint and T-Mobile networks distinguishable. \label{fig:cdf_cities_dbs}

Figure~\ref{fig:cdf_cities_dbs} shows accuracies observed in New York, Chicago, and Philadelphia
  for major broadband carriers in each market.
In the best cases, such as either RCN or Comcast on MaxMind in Chicago,
  the median error is less than 5~km.
In each city/database pair, the accuracy is good for fixed broadband
  and poor for any mobile broadband.
In Chicago, MaxMind is more accurate with RCN, WOW, and Comcast than mixed (AT\&T)
  and pure mobile (T-Mobile, Sprint, Verizon) carriers.
(IP2Location performs poorly with RCN.)
Similarly in New York, Charter, Cablevision, and Comcast are better localized than AT\&T, Sprint, T-Mobile, and Verizon;
  and in Philadelphia, geolocation is more accurate on Comcast than Verizon (which offers both fixed and mobile),
  T-Mobile or AT\&T (mobile only).

Quantitatively, the share of Comcast addresses in New York 
  that MaxMind locates within 10~km of the GPS location is 66\%.
At the other extreme, 88\% of T-Mobile addresses from the New York region 
	are assigned to just two distinct locations representing New York itself and Newark;
	99\% are assigned either to those two, or 
    to one of six other locations in Philadelphia (3), Providence, Boston, and Washington.
As a result, only 17\% of devices are assigned within 10~km of their true location.
In fairness, it must be emphasized that MaxMind does not \emph{claim} to 
  assign these devices within 10~km: almost all of the T-Mobile addresses assigned to the New York and Newark
	locations are in the 200~km accuracy class.

This basic dichotomy between mobile and fixed broadband
	is apparent even within ISPs.
AT\&T offers both services in Chicago, and its CDF is notably different from other 
	mobile providers at high accuracy / low error.
Indeed, we can confirm that the subnets with 
	the largest geolocation errors belong to the AT\&T Mobility organization.
By contrast, AT\&T in New York and Philadelphia is purely wireless,
	which is reflected in those cumulative distributions.
This observation once stated, 
  perhaps appears obvious, but it need not have been true.
Mobile carriers could have constructed networks so that individual antennas
  held a fixed set of IP addresses.
That does not appear to be what they did.

Before continuing, we also contrast geolocation performance on 
  consumer fixed-broadband, with large universities and companies.
We include Universities with at least ten thousand students,
  and Fortune 100 companies other than ISPs.
Again, we note that we are implicitly studying the WiFi
  access points that these institutions operate and which 
  their employees, students, and clients connect to via mobile devices,
  rather than fixed infrastructures of servers.
Universities are a classic geolocation target,
  but Figure~\ref{fig:f100_edu} shows that they are
  in general more-accurately geolocated than either 
  consumer ISPs or companies.
This is not surprising: they have large, physically-concentrated networks,
  with registration addresses clearly spelled out in ARIN records.
In most cases, median geolocation error is less than 2~km,
  though a few institutes -- DePaul in Chicago and the City University of New York --
  are mislocated by upwards of 10~km.

cdf_cities_dbs_cats.pdf:1.0 Geolocation performance on consumer ISPs, contrasted with large universities and Fortune 100 companies. \label{fig:f100_edu}

Figures \ref{fig:cdf_by_city}-\ref{fig:f100_edu}
  suggest that for a substantial share of IP addresses,
  IP geolocation is quite accurate. 
However, this does not do us much good unless those locations
  can be identified in advance.
It is already clear that the picture is rosier with fixed broadband.
Those data can be easily identified,
  either via a \texttt{whois} look-up or (in some cases)
  through the geolocation databases themselves.
But mobile and fixed is not the only lever.
MaxMind is able to perform better on RCN than on Comcast in Chicago,
  and better on Charter or Cablevision than Comcast in New York.
How are we to identify localizable blocks of addresses?

We highlight two additional methods.
MaxMind's database provides an “accuracy” field that successfully 
  identifies the precision of entries.
Figure~\ref{fig:cdf_mm_by_accuracy} shows the CDF for 
  successive bins of claimed accuracy.
In the most precise bin, accuracy of “1~km,”
  the median device in Chicago is geolocated just 2.1~km
  from the GPS-based location.
The “error” with respect to the ground-truth 
  degrades in-line with quoted accuracy,
	though there is enormous spread in the least-precise, 500~km bin.
It is thus \emph{possible} to identify 
  accurately-located addresses -- MaxMind does it.
But this leaves an open question:
  \emph{why} are those addresses well or ill-located?

That brings us to the second method.
Our hypothesis is that 
  if /24 subnets are geographically localized~-- small~--
  then addresses within them are more-likely to be accurately geolocated.
If they are large, then precise locations would require finer address-level data.
The question can then be re-posed:
  how large are subnets, and is their size in fact correlated with geolocation accuracy?

cdf_mm_by_accuracy.pdf:0.6 Cumulative distribution of geolocation accuracy on the MaxMind database, by quoted accuracy bin.  \label{fig:cdf_mm_by_accuracy}

>> How large are /24 subnets?
What are the physical and network properties of accurately-located subnets?
We focus this analysis on a single, fixed network~-- Comcast~-- 
  and require that subnets have at least 10 devices and 10 distinct IP addresses;
There are over twenty thousand such subnets between the three cities.

To quantify whether or not a subnet is localized,
   we define a characteristic physical scale.
Many subnets have some outliers,
  perhaps with locations reported after the fact.
To mitigate the impact of these outliers,
  we must first identify them.
We compute the medioid of locations in the subnet, 
  defined in this case simply as the median of the $x$ and $y$ coordinates 
  in a projected (flat) geometry (EPSG 2163).
We then measure individual locations' distances from that medioid.
We select a configurable fraction $f$ of the data that is “closest” by that measure.
For that subset of the data, we calculate the convex hull.
If $f = 1$, then the convex hull covers all locations recorded on the subnet;
  if $f = 1/2$, it covers the half of points closest to the medioid.
Finally we take the area of the convex hull,
  and “convert” this area to a distance by taking its square root.
That square root defines the length scale of the subnet.
Figure~\ref{fig:convex_hull} illustrates this procedure for two subnets.
(To preserve anonymity,
  random noise has been added to the individual points in the illustration.)

convex_hull.png:0.7 Convex hulls constructed for one dispersed and one well-localized subnet in Chicago.  The linear scale on the right-hand side (67.176.158.0/24) is a factor of 8 larger than on the right-hand side.  Gaussian noise has been added to the locations for illustrative purposes only.  The convex hull is constructed to cover $f = 0.9$ of the input points in the subnet. \label{fig:convex_hull}

Figure~\ref{fig:subnet_scale} shows this distance scale
  for subnets with at least 10 devices and addresses, 
  for several choices of $f$.
Clearly, the scale is smaller or larger when outliers are more or less suppressed.
Setting $f = 0.5$ results in a median subnet scale of 3~km,
  and $f = 0.9$ leads to a scale of 8~km.
The proportion of subnets with scales exceeding 10~km is small, for any choice of $f$.

subnet_scale.pdf:0.55; scale_nvisits.pdf:0.45; Cumulative density of subnets' distance scale as derived from the convex hull of locations, as described in the text.  At right, the number of times an a single device visits a single IP address on the subnet (weighted by visits).  On subnets with scale greater than 20~km ($f = 0.75$), over half of visits device/IP pairs are unique. \label{fig:subnet_scale}

Armed with this scale, we return to the earlier question: 
  when can subnets be accurately located?
Discarding locations with geolocation error over 100~km, 
  the correlation between subnet scale and mean geolocation error,
  is 0.62 for MaxMind but only 0.24 on IP2Location (which has worse overall performance).
We confirm the hypothesis that localization and localizability are indeed related, 
  though strictly speaking, this analysis is not causal.

Still, this analysis has postponed,
  but not \emph{answered} the question;
  it suggests why geolocation fails on certain subnets of fixed providers,
  but leaves open why the large subnets exist at all.
Comcast uses both large and small subnets;
  do they use the large ones differently?
Taking a hint from the results on mobile broadband,
  we hypothesize that the small subnets are nearly static 
  whereas large ones provide ``ephemeral" addresses~--
    perhaps while waiting for a static one to be assigned.
A client assigned to an ``ephemeral" address
  would be unlikely to fall on that same address again,
  whereas a ``sticky" address granted to a home network would be used repeatedly.
The relevant variable is thus the number of times
  that a single client is observed at each IP address
  (weighted by visits).
The right-hand side of Figure~\ref{fig:subnet_scale}
  confirms this hypothesis:
  for subnets with scale greater than 20~km ($f = 0.75$)
  most visitors to an IP address visit exactly once.


>> How rapidly do subnets on fixed-broadband networks move?

Geolocation providers are quick to point out that
  their databases evolve continuously.
Clearly, the physical infrastructure of the Internet evolves over time,
  but how quickly do subnets actually move?

Figure~\ref{fig:movement_by_month} presents
  the distance moved by /24 subnet medioids between August and October 2020.
To enter into this figure, subnets must have at least ten unique devices
  and ten unique addresses in each month.
We consider only fixed-broadband carriers, for this exercise.
On Charter, Cablevision, and RCN,
  the median subnet moves less than a kilometer;
  on Comcast, the median is less than two kilometers.
In other words, on the two-month time scale, there is very little movement.

movement_by_month.pdf Displacement of /24 subnet medioids over a two-month period from August to October 2020, for fixed broadband providers.  \label{fig:movement_by_month}

A substantial threat to this analysis is sample composition:
  by requiring 10 devices and 10 addresses,
  the subnet \emph{must} be observed in New York, Chicago, or Philadelphia
  in both months, to enter the sample at all.
However, it does not seem to be the case that subnets are moving out of sample.
Of the subnets satisfying the cuts in August, 92\% also pass them in October (vice versa, 96\%).
If we raise the thresholds to enter the sample, requiring 20 devices and 20 addresses,
  95\% of subnets passing these cuts in August also show up with at least 10 devices in October (vice versa, 98\%).
Raising the thresholds yet further to 50 devices and 50 addresses,
  the persistence from August to October exceeds 99\% (vice versa, 98\%).

> Implications for Demographic Research

Before concluding, we return to the question that initially motivated this research:
  can IP geolocation be used to link data on Internet performance and use with human populations?
\emph{Where} and \emph{for what demographic groups} is geolocation accurate?
To make this query concrete, imagine a study of the ``homework gap" --  
  (in)equity in access to digital resources for education --
  based solely on server logs from a site like Wikipedia.
If we observe frequencies of use by IP subnet \emph{alone},
  can we infer what groups do and do not access the site?

This question is non-trivial, 
  since it confronts the correlations of 
  population density and demographics with geolocation accuracy,
  along with the spatial patterns of connection modality (mobile vs fixed).
Cities have smaller subnets simply 
  because they have higher density of people and devices.
They also tend to have larger minority populations.
This alone leads to a correlation between geolocation accuracy with 
  demographics or disadvantage.
For Chicago and its buffer, 
  the correlation between tract
  median geolocation error on MaxMind and population density is $-0.07$ ($p < 0.0005$);
  in turn, population density is correlated with log median household income
    ($r = -0.18$, $p < 10^-10$).
Both of these are small but significant.
The flip side of better accuracy at higher density 
  is that distance precision \emph{has} to improve
  in dense environments, to associate activity with the right population.
It's easier to ``jump" over many people when they are close together.

Accuracy also varies \emph{within} the city, 
  due to heterogeneity in the fraction of 
  people on mobile vs fixed broadband.
There are two reasons for this.
People use mobile devices (1) when they are on the go,
  or (2) because they do not have access to a fixed broadband connection at home.
That means that devices in the present sample observed in city centers
  appear to have ``inaccurate" IP geolocation,
  simply because the device users are more-likely on mobile on the way to or at work.\fnote{Appendix: Add table of MaxMind accuracy at all times (to show daily trends)?}
On the other hand, 
  populations without fixed broadband access 
  are unlikely to be accurately IP geolocated, even in their home neighborhood.

As a final consideration before proceeding, 
  one must not confound ``unknown" addresses with ``mis-located" ones.
For example, if a default database location for T-Mobile addresses sits in a particular neighborhood,
  that neighborhood will appear to have ``accurate" geolocation, even though 
  the locations are not known any better than elsewhere.
Performance will appear to ``degrade" radially, with distance from the default location.
Since the default locations are usually in or near cities,
  that would (\emph{ceteris paribus}) give a false impression
  that IP addresses in cities (or near the geographic center of the United States, or ``Null Island")
  are accurately-located.

Turning to the data, Figure~\ref{fig:chicago_mobile} presents the proportion of the night-time clusters in 
  each tract of Chicago, that are on fixed and mobile broadband.
Note that the data are inherently mobile devices with GPS chips; 
  this does not include laptops, for instance.
This defines Comcast, WOW, and RCN, as fixed, 
  and T-Mobile, Sprint, Verizon, and AT\&T as mobile.
(The classification for AT\&T is ambiguous; 
  similar results are obtained if those data are simply dropped.)
For those familiar with Chicago, the results are no surprise:
  the proportion of night-time pings on mobile networks
  is lower on the wealthier North Side of the city than on the West or South Sides.
Indeed, our eyes do not deceive us:
  the tract level correlation between this constructed variable
  and share of households with a broadband contract as reported to the Census is $-0.25$.
The correlation to neighborhood proportion Hispanic is $0.23$ (both $p < 10^{-10}$).
In other words, connection type is correlated with demographic factors and broadband adoption.
This would be reflected in geolocation accuracy.
In practice,
  this means that constraining an analysis to accurately-located, fixed-broadband IP addresses
  would tend to exclude vulnerable populations from the analysis.

chicago_mobile.pdf Proportion of night-time clusters in Chicago recorded on mobile networks.  \label{fig:chicago_mobile}

Figure~\ref{fig:race_ethn_cdf}
  offers an alternative view of this effect,
  disentangling the countervailing forces of density,
    demographics, and access modality.
It displays the CDF of device geolocation accuracy for hyper-segregated neighborhoods of Chicago~--
  ones where two-thirds of residents are white (only), Black (alone or in combination with other races), or Hispanic (of any race).
Moving from left to right, 
  we begin from the full dataset and layer the cumulative
  requirements of devices in Chicago proper (not the 40 mile buffer), 
  at night (that is, likely at home), and 
  on Comcast (i.e., on a single, fixed broadband network).
The first plot shows an enormous difference between geolocation in ``white" tracts and other segregated tracts -- 
  geolocation performs much worse.
This effect appears to have more to do with density than race:
  it reverses when focusing on the City of Chicago,
  and zeroing in on a single network, the performance lines up quite closely.
The exception is at the very high end (above 10~km and 90\% of the CDF),
  where there is apparently an error for a set of white tracts.
About 80\% of points are within 5~km of the true location, for all three categories of neighborhood.

race_ethn_cdf.pdf:1.0 Cumulative distribution of geolocation error for tracts with white, Black, and Hispanic super-majorities.  The first panel presents all data, while the second through fourth restrict to Chicago, Chicago at night, and Chicago at night on Comcast.  \label{fig:race_ethn_cdf}

The analyses above suggest that IP geolocation databases'
  ability to attribute online behaviors to populations will tend to fail more often for disadvantaged groups.
Still, if we were to persist, what errors might we expect to ``accrue," by moving an 
  observation from its GPS-based location to the IP-based location?
In essence, this question pits the scale of geolocation accuracy against
  the physical scale of demographic segregation.
If IP geolocation moves a point among communities with similar
  demographics, the error does not directly bias results.
This analysis is limited to fixed-broadband data from Comcast,
  where geolocation has a chance of succeeding.
Figure~\ref{fig:log_mhi_quantiles} presents the log median household income as it would be imputed from a MaxMind look-up,
  against the true median household income of the neighborhood (Census tract).
This results in an unsurprising regression to the mean:
  as is the usual case with measurement error, the slope is simply attenuated.
This suggests that even for fixed broadband,
  efforts to using IP address alone to ``link" online behaviors with human populations are inadvisable.
They will in general yield estimates whose magnitudes are biased down.
In other words, measurements of ``who uses what"
  that rely on IP geolocation will tend to \emph{understate} differential access.

log_mhi_quantiles.pdf Quantiles of neighborhood log median household income as ``imputed'' from MaxMind geolocation ($y$) as a function of the true neighborhood value ($x$). \label{fig:log_mhi_quantiles}


% median_error_by_geoid:1.0 Median geolocation error on MaxMind, by Census Tract. \label{fig:median_error_by_geoid}


> Conclusions

Using a large sample of GPS-based smartphone lcoations
  this paper has quantified the performance of commercial geolocation databases
  in large American cities.
The precision of this analysis far outstrips past work.
The analysis has demonstrated significant heterogeneity in geolcoation accuracy.
The median error for MaxMind's free service is well less than 10~km, on 
  fixed commercial broadband networks and at Universities.
Geolocation accuracy is adequate only for city-level wor
On mobile networks, IP geolocation is not accurate below the city level.

This analysis has also sought to explain \emph{why} some addresses
  are accurately located whereas others are not.
The physical size of subnets is strongly correlated with accuracy.
Large subnets appear to be used for ``ephemeral" address assignment, 
  which clients do not use repeatedly.

Finally, we have contextualized these findings for applications to research on human populations.
Both the present data and existing surveys show that 
  disadvantaged populations are less likely to use a fixed broadband subscription at home.
Online behaviors cannot be accurately associated with these groups,
  and dropping mobile devices altogether will tend to remove them from analyses.
Focussing on the context where geolocation does work -- fixed-line broadband~-- 
  the accuracy still appears inadequate for associating online activities
  with real-world geographies and demographics.
From a privacy perspective, a single IP address does not identify an individual,
  but it both localizes and individual and provides 
  an ``index" through time that may be used to aggregate other indirect identifiers.


> To-Do

- Add paid versions of databases
- Wireless breakouts for AT\&T and Verizon
- Re-run data, dropping 2-decimal precisoin and foreign NICs
- August only
- How long does a device stay on the same IP at night?

\bibliographystyle{bibulous_natbib}
\bibliography{sources}

\clearpage
\appendix

\input{tabs/unacast_classification_freq.tex}

\input{tabs/foreign_nic_fracs.tex}

travel_no_travel.pdf Empirical cumulative distribution for \label{fig:travel_no_travel}

cdf_chicago_ookla.pdf; Geolocation error of GPS location targets in Chicago, on both Unacast and Ookla Speedtest Intelligence data.

ookla_subnet_scale.pdf:0.65; Subnet scale measured using Ookla speedtest data. \label{fig:subnet_scale_ookla}



==> tabs/distance_quantiles_by_db.tex <==
\begin{table}
\centering
\caption{Quantiles of accuracy for both databases, in kilometers. \label{tab:distance_quantiles_by_db}}
\begin{tabular}{crr}
\toprule
 Quantile &  MaxMind &  IP2Location \\
\midrule
     0.10 &      2.6 &          7.1 \\
     0.25 &      9.3 &         17.5 \\
     0.50 &     27.0 &         46.5 \\
     0.75 &     56.2 &        148.8 \\
     0.90 &    122.2 &        477.2 \\
\bottomrule
\end{tabular}
\end{table}

